Characterizing Interest Aggregation in Content-Centric Networks

The Named Data Networking (NDN) and Content-Centric Networking (CCN) architectures advocate Interest aggregation as a means to reduce end-to-end latency and bandwidth consumption. To enable these benefits, Interest aggregation must be realized through Pending Interest Tables (PIT) that grow in size at the rate of incoming Interests to an extent that may eventually defeat their original purpose. A thorough analysis is provided of the Interest aggregation mechanism using mathematical arguments backed by extensive discrete-event simulation results. We present a simple yet accurate analytical framework for characterizing Interest aggregation in an LRU cache, and use our model to develop an iterative algorithm to analyze the benefits of Interest aggregation in a network of interconnected caches. Our findings reveal that, under realistic assumptions, an insignificant fraction of Interests in the system benefit from aggregation, compromising the effectiveness of using PITs as an integral component of Content-Centric Networks.

==> bib/biblio.tex <==

@INPROCEEDINGS{ghodsi:11,
  title = "{Information-Centric Networking: Seeing the Forest for the Trees}",
  author_ = {Ghodsi, Ali and Shenker, Scott and Koponen, Teemu and Singla, Ankit and Raghavan, Barath and Wilcox, James},
  author = {Ghodsi~\etal, Ali},
  booktitle = {Proc. ACM HotNets},
  pages = {1--6},
  month_ = nov,
  year = {2011},
  address = {Cambridge, MA}
}

@ARTICLE{fayazbakhsh:13,
  title = "{Less Pain, Most of the Gain: Incrementally Deployable ICN}",
  author_ = {Fayazbakhsh, Seyed and Lin, Yin and Tootoonchian, Amin and Ghodsi, Ali and Koponen, Teemu and Maggs, Bruce and Ng, K. and Sekar, Vyas and Shenker, Scott},
  author = {Fayazbakhsh~\etal, Seyed},
  journal = {ACM SIGCOMM Comput. Commun. Rev.},
  journal_ = {ACM SIGCOMM Computer Communication Review},
  volume = {43},
  number = {4},
  pages = {147--158},
  month_ = oct,
  year = 2013,
}

@ARTICLE{dan:90,
 author = {Dan, Asit and Towsley, Don},
 title = "{An Approximate Analysis of the LRU and FIFO Buffer Replacement Schemes}",
 journal = {ACM SIGMETRICS Perform. Eval. Rev.},
 journal_ = {ACM SIGMETRICS Performance Evaluation Review},
 volume = {18},
 number = {1},
 month_ = apr,
 year = {1990},
 pages = {143--152},
}

@ARTICLE{che:02,
  title = "{Hierarchical Web Caching Systems: Modeling, Design and Experimental Results}",
  author_ = {Che, Hao and Tung, Ye and Wang, Zhijun},
  author = {Che~\etal, Hao},
  journal = {IEEE J. Sel. Areas Commun.},
  journal_ = {IEEE Journal on Selected Areas in Communications},
  volume = {20},
  number = {7},
  month_ = sep,
  pages = {1305--1314},
  year = {2002},
}

@INPROCEEDINGS{fricker:12itc,
  title = "{A Versatile and Accurate Approximation for LRU Cache Performance}",
  author_ = {Fricker, Christine and Robert, Philippe and Roberts, James},
  author = {Fricker~\etal, Christine},
  booktitle = {Proc. ITC},
  booktitle_ = {Proc. International Teletraffic Congress},
  pages = {1--8},
  month_ = sep,
  year = {2012},
  address = {Krakow, Poland},
}

@ARTICLE{kurose:14,
  title = "{Information-Centric Networking: The Evolution from Circuits to Packets to Content}",
  journal = {Comput. Netw.},
  journal_ = {Computer Networks},
  volume = 66,
  number = 0,
  pages = {112--120},
  year = {2014},
  month_ = jun,
  author = {Jim Kurose},
}

@ARTICLE{ahlgren:12,
  title = "{A Survey of Information-Centric Networking}",
  author_ = {Ahlgren, Bengt and Dannewitz, Christian and Imbrenda, Claudio and Kutscher, Dirk and Ohlman, B{\"o}rje},
  author = {Ahlgren~\etal, Bengt},
  journal = {IEEE Commun. Mag.},
  journal_ = {IEEE Communications Magazine},
  volume = {50},
  number = {7},
  pages = {26--36},
  year = {2012},
  month_ = jul,
}

@MISC{ccnx,
  title_ = "{Content Centric Networking Project (CCN)}",
  url = {http://www.ccnx.org/},
  originalyear_ = {2014-04-01},
  note_ = {Accessed: 2015-07-27},
}

@MISC{squid,
  url = {http://www.squid-cache.org},
}

@ARTICLE{koponen:07,
  title = "{A Data-Oriented (and Beyond) Network Architecture}",
  author_ = {Koponen, Teemu and Chawla, Mohit and Chun, Byung and Ermolinskiy, Andrey and Kim, Kye and Shenker, Scott and Stoica, Ion},
  author = {Koponen~\etal, Teemu},
  journal = {ACM SIGCOMM Comput. Commun. Rev.},
  journal_ = {ACM SIGCOMM Computer Communication Review},
  volume = {37},
  number = {4},
  pages = {181--192},
  year = {2007},
  month_ = aug,
}

@INPROCEEDINGS{jacobson:09,
  title = "{Networking Named Content}",
  author_ = {Jacobson, Van and Smetters, Diana and Thornton, James and Plass, Michael and Briggs, Nicholas and Braynard, Rebecca },
  author = {Jacobson~\etal, Van},
  booktitle = {Proc. ACM CoNEXT},
  pages = {1--12},
  year = {2009},
  month_ = dec,
  address = {Rome, Italy}
}

@ARTICLE{dannewitz:13,
  title = "{Network of Information (NetInf)--An Information-Centric Networking Architecture}",
  author_ = {Dannewitz, Christian and Kutscher, Dirk and Ohlman, B{\"o}rje and Farrell, Stephen and Ahlgren, Bengt and Karl, Holger},
  author = {Dannewitz~\etal, Christian},
  journal = {Comput. Commun.},
  journal_ = {Computer Communications},
  volume = {36},
  number = {7},
  pages = {721--735},
  year = {2013},
  month_ = apr,
}

@ARTICLE{zhang:14,
  title = "{Named Data Networking}",
  author_ = {Zhang, Lixia and Afanasyev, Alexander and Burke, Jeffrey and Jacobson, Van and kc claffy and Crowley, Patrick and Papadopoulos, Christos and Wang, Lan and Zhang, Beichuan},
  author = {Zhang~\etal, Lixia},
  journal = {ACM SIGCOMM Comput. Commun. Rev.},
  journal_ = {ACM SIGCOMM Computer Communication Review},
  volume = 44,
  number = 3,
  pages = {66--73},
  year = 2014,
}

@INPROCEEDINGS{roberts:13,
  title = "{Exploring the Memory-Bandwidth Tradeoff in an Information-Centric Network}",
  author = {Roberts, James and Sbihi, Nada},
  booktitle = {Proc. ITC},
  pages = {1--9},
  year ={2013},
  month_ = sep,
  address = {Shanghai, China}
}

@INPROCEEDINGS{carofiglio:11,
  title = "{Bandwidth and Storage Sharing Performance in Information Centric Networking}",
  author_ = {Carofiglio, Giovanna and Gallo, Massimo and Muscariello, Luca},
  author = {Carofiglio~\etal, Giovanna},
  booktitle = {Proc. ACM SIGCOMM Workshop on ICN},
  pages = {26--31},
  year = {2011},
  month_ = aug,
  address = {Toronto, Canada}
}

@INPROCEEDINGS{carofiglio:itc11,
  title = "{Modeling Data Transfer in Content-Centric Networking}",
  author_ = {Carofiglio, Giovanna and Gallo, Massimo and Muscariello, Luca and Perino, Diego},
  author = {Carofiglio~\etal, Giovanna},
  booktitle = {Proc. ITC},
  pages = {111--118},
  year = {2011},
  month_ = sep,
  address_ = {San Francisco, CA, USA},
  address = {San Francisco, USA},
}

@INPROCEEDINGS{rosensweig:10,
  title = "{Approximate Models for General Cache Networks}",
  author_ = {Rosensweig, Elisha and Kurose, Jim and Towsley, Don},
  author = {Rosensweig~\etal, Elisha},
  booktitle = {Proc. IEEE INFOCOM},
  pages = {1--9},
  year = {2010},
  month_ = mar,
  address_ = {San Diego, CA, USA},
  address = {San Diego, USA}
}

@BOOK{daley:03,
  title = "{An Introduction to the Theory of Point Processes}",
  author = {Daley, Daryl and Vere-Jones, David},
  volume = {I: Elementary Theory and Methods},
  edition = {Second},
  year = {2003},
  publisher = {Springer},
  address_ = {New York, NY, USA},
  address = {New York, USA},
}

@ARTICLE{hawkes:71,
  title = "{Spectra of Some Self-Exciting and Mutually Exciting Point Processes}",
  author = {Hawkes, Alan},
  journal_ = {Biometrika},
  volume = {58},
  number = {1},
  pages = {83--90},
  year = {1971},
  month_ = apr,
}

@INPROCEEDINGS{gill:07,
  title = "{Youtube Traffic Characterization: A View from the Edge}",
  author_ = {Gill, Phillipa and Arlitt, Martin and Li, Zongpeng and Mahanti, Anirban},
  author = {Gill~\etal, Phillipa},
  booktitle = {Proc. ACM IMC},
  pages = {15--28},
  year = {2007},
  month_ = oct,
  address_ = {San Diego, CA, USA},
  address = {San Diego, USA}
}

@INPROCEEDINGS{rosensweig:13,
  title = "{On the Steady-State of Cache Networks}",
  author_ = {Rosensweig, Elisha and Menasche, Daniel and Kurose, Jim},
  author = {Rosensweig~\etal, Elisha},
  booktitle = {Proc. IEEE INFOCOM},
  pages = {863--871},
  year = {2013},
  month_ = apr,
  address = {Turin, Italy}
}

@INPROCEEDINGS{wang:13, 
  author_ = {Yonggong Wang and Zhenyu Li and Tyson, G. and Uhlig, S. and Gaogang Xie}, 
  author = {Yonggong Wang~\etal}, 
  booktitle = {Proc. IEEE ICNP},
  booktitle_ = {Proc. IEEE International Conference on Network Protocols},
  title = "{Optimal Cache Allocation for Content-Centric Networking}", 
  year = {2013},
  month_ = oct, 
  pages = {1--10},
  address = {G{\"o}ttingen, Germany}
}

@ARTICLE{jelenkovic:04,
  title = "{Least-Recently-Used Caching with Dependent Requests}",
  author = {Jelenkovi{\'c}, Predrag and Radovanovi{\'c}, Ana},
  journal = {Theor. Comput. Sci.},
  journal_ = {Theoretical Computer Science},
  volume = {326},
  number = {1},
  pages = {293--327},
  year = {2004},
  month_ = oct,
}

@ARTICLE{rodriguez:01,
  title = "{Analysis of Web Caching Architectures: Hierarchical and Distributed Caching}",
  author_ = {Rodriguez, Pablo and Spanner, Christian and Biersack, Ernst},
  author = {Rodriguez~\etal, Pablo},
  journal = {IEEE/ACM Trans. Netw.},
  journal_ = {IEEE/ACM Transactions on Networking},
  volume = {9},
  number = {4},
  pages = {404--418},
  year = {2001},
  month_ = aug,
}

@INCOLLECTION{psaras:11,
  title = "{Modelling and Evaluation of CCN-Caching Trees}",
  author_ = {Psaras, Ioannis and Clegg, Richard and Landa, Raul and Chai, Wei and Pavlou, George},
  author = {Psaras~\etal, Ioannis},
  booktitle = {Proc. IFIP Networking},
  pages = {78--91},
  year = {2011},
  month_ = may,
  location = {Valencia, Spain},
  publisher={Springer}
}

@INCOLLECTION{chai:12,
  title = " {Cache ``Less for More'' in Information-Centric Networks}",
  author_ = {Chai, Wei and He, Diliang and Psaras, Ioannis and Pavlou, George},
  author = {Chai~\etal, Wei},
  booktitle = {Proc. IFIP Networking},
  pages = {27--40},
  year = {2012},
  month_ = may,
  location = {Prague, Czech Republic},
  publisher = {Springer},
}

@ARTICLE{chai:13,
  title = "{Cache ``Less for More'' in Information-Centric Networks (Extended Version)}",
  author_ = {Chai, Wei and He, Diliang and Psaras, Ioannis and Pavlou, George},
  author = {Chai~\etal, Wei},
  journal = {Comput. Commun.},
  journal_ = {Computer Communications},
  volume = {36},
  number = {7},
  pages = {758--770},
  year = {2013},
  month_ = apr,
}

@INPROCEEDINGS{psaras:12,
  title = "{Probabilistic In-Network Caching for Information-Centric Networks}",
  author_ = {Psaras, Ioannis and Chai, Wei and Pavlou, George},
  author = {Psaras~\etal, Ioannis},
  booktitle = {Proc. ACM SIGCOMM Workshop on ICN},
  pages = {55--60},
  year = {2012},
  month_ = aug,
  address = {Helsinki, Finland}
}

@ARTICLE{Gallo:14,
  title = "{Performance Evaluation of the Random Replacement Policy for Networks of Caches}",
  author_ = {Massimo Gallo and Bruno Kauffmann and Luca Muscariello and Alain Simonian and Christian Tanguy},
  author = {Massimo Gallo~\etal},
  journal = {Perform. Evaluation},
  journal_ = {Performance Evaluation},
  volume = {72},
  number = {0},
  pages = {16--36},
  year = {2014},
  month_ = feb,
} 

@ARTICLE{melazzi:14,
  title = "{A General, Tractable and Accurate Model for a Cascade of LRU Caches}",
  author_ = {Melazzi, N and Bianchi, G and Caponi, A and Detti, A},
  author = {Melazzi~\etal, N},
  journal = {IEEE Commun. Lett.},
  journal_ = {IEEE Communications Letters},
  volume = {18},
  number = {5},
  pages = {877--880},
  year = {2014},
  month_ = may,
}

@INPROCEEDINGS{martina:14,
  title = "{A Unified Approach to the Performance Analysis of Caching Systems}",
  author_ = {Valentina Martina and Michele Garetto and Emilio Leonardi},
  author = {Valentina Martina~\etal},
  booktitle = {Proc. IEEE INFOCOM},
  pages = {2040--2048},
  month_ = apr,
  year = {2014},
  address = {Toronto, Canada},
}

@INPROCEEDINGS{tyson:12,
  title = "{A Trace-Driven Analysis of Caching in Content-Centric Networks}",
  author_ = {Tyson, Gareth and Kaune, Sebastian and Miles, Simon and El-khatib, Yehia and Mauthe, Andreas and Taweel, Adel},
  author = {Tyson~\etal, Gareth},
  booktitle = {Proc. ICCCN},
  pages = {1--7},
  year = {2012},
  month_ = jul,
  address = {Munich, Germany}
}

@ARTICLE{danzig:93,
 author_ = {Danzig, Peter and Hall, Richard and Schwartz, Michael},
 author = {Danzig~\etal, Peter},
 title = "{A Case for Caching File Objects Inside Internetworks}",
 journal = {SIGCOMM Comput. Commun. Rev.},
 journal_ = {ACM SIGCOMM Computer Communication Review},
 volume = {23},
 number = {4},
 month_ = oct,
 year = {1993},
 pages = {239--248},
} 

@INPROCEEDINGS{rossi:12, 
  author = {Rossi, D. and Rossini, G.}, 
  booktitle = {Proc. IEEE INFOCOM Workshops}, 
  title = "{On Sizing CCN Content Stores by Exploiting Topological Information}", 
  year = {2012},
  month_ = mar, 
  pages = {280--285},
  address_ = {Orlando, FL, USA},
  address = {Orlando, USA},
}

@TECHREPORT{rossi:11,
  author = {Rossi, Dario and Rossini, Giuseppe},
  title = "{Caching Performance of Content Centric Networks Under Multi-Path Routing (and More)}",
  institution = {Telecom ParisTech},
  year = 2011,
  type = {Technical Report},
}

@INPROCEEDINGS{fonseca:03,
  author_ = {Fonseca, R. and Almeida, V. and Crovella, M. and Abrahao, B.}, 
  author = {Fonseca~\etal, R.}, 
  booktitle = {Proc. IEEE INFOCOM}, 
  title = "{On the Intrinsic Locality Properties of Web Reference Streams}", 
  year = {2003}, 
  month_ = mar, 
  pages = {448--458},
  address_ = {San Francisco, CA, USA},
  address = {San Francisco, USA},
}

@ARTICLE{cherkasova:04,
  title = "{Analysis of Enterprise Media Server Workloads: Access Patterns, Locality, Content Evolution, and Rates of Change}",
  author = {Cherkasova, Ludmila and Gupta, Minaxi},
  journal = {IEEE/ACM Trans. Netw.},
  journal_ = {IEEE/ACM Transactions on Networking},
  volume = {12},
  number = {5},
  pages = {781--794},
  year = {2004},
  month_ = oct,
}

@TECHREPORT{ndnSIM,
  author_ = {Alexander Afanasyev and Ilya Moiseenko and Lixia Zhang},
  author = {Afanasyev~\etal, Alexander},
  title = "{ndnSIM: NDN Simulator for NS-3}",
  institution = {NDN},
  year = {2012},
  type = {Technical Report},
  number = {NDN-0005},
  month_ = oct,
  url = {http://named-data.net/techreports.html},
}

@UNPUBLISHED{domingues:13,
  title = "{Enabling Information Centric Networks through Opportunistic Search, Routing and Caching}",
  author = {Guilherme Domingues and Edmundo Silva and Rosa Le{\~a}o and Daniel Menasch{\'e}},
  month_ = oct,
  year = {2013},
  note = {arXiv:1310.8258 [cs.NI]},
}

@ARTICLE{cinlar:68,
  title = "{On the Superposition of Point Processes}",
  author = {Cinlar, E and Agnew, R},
  journal = {J. Roy. Stat. Soc. B Met.},
  journal_ = {Journal of the Royal Statistical Society. Series B (Methodological)},
  volume = {30},
  number = {3},
  pages = {576--581},
  year = {1968}, 
}

@INCOLLECTION{cao:03,
  title = "{Internet Traffic Tends Toward Poisson and Independent as the Load Increases}",
  author_ = {Cao, Jin and Cleveland, William and Lin, Dong and Sun, Don},
  author = {Cao~\etal, Jin},
  booktitle = {Lect. Notes. Stat.},
  series_ = {},
  booktitle_ = {Nonlinear Estimation and Classification},
  series_ = {Lecture Notes in Statistics},
  pages = {83--109},
  year = {2003},
  volume = {171},
  publisher = {Springer New York},
}

@MISC{caida,
  title = "{Internet Topology at Router- and AS-levels}",
  url = {http://www.caida.org/research/topology/generator},
  originalyear = {2013-11-07},
  note = {Accessed: 2015-07-17},
}

@MISC{russakovskii:08,
  title = "{How to Find Out the Number of Videos on Youtube}",
  author = {Artem Russakovskii},
  url = {http://beerpla.net/2008/08/14/how-to-find-out-the-number-of-videos-on-youtube/},
  year = {2008},
  note = {Accessed: 2015-07-22},
}

@INPROCEEDINGS{fricker:12infocom, 
  author_ = {Fricker, C. and Robert, P. and Roberts, J. and Sbihi, N.}, 
  author = {Fricker~\etal, C.}, 
  booktitle = {Proc. IEEE INFOCOM Workshops}, 
  title = "{Impact of Traffic Mix on Caching Performance in a Content-Centric Network}", 
  year = 2012, 
  month_ = mar, 
  pages = {310--315},
  address_ = {Orlando, FL, USA},
  address = {Orlando, USA},
}

@ARTICLE{mahanti:00, 
  author_ = {Mahanti, A. and Williamson, C. and Eager, D.}, 
  author = {Mahanti~\etal, A.}, 
  journal_ = {IEEE Network}, 
  journal = {IEEE Netw.}, 
  title = "{Traffic Analysis of a Web Proxy Caching Hierarchy}", 
  year = {2000}, 
  month_ = may,
  volume = {14}, 
  number = {3}, 
  pages = {16--23}, 
}

@PHDTHESIS{fraleigh:02,
  author = {Fraleigh, Charles}, 
  title = "{Provisioning Internet Backbone Networks to Support Latency Sensitive Applications}",
  school = {Stanford University},
  year = 2002,
  address_ = {Stanford, CA, USA},
  address = {Stanford, USA},
  month_ = may,
}

@ARTICLE{cowie:99,
  title = "{Modeling the Global Internet}",
  author_ = {Cowie, James and Nicol, David and Ogielski, Andy},
  author = {Cowie~\etal, James},
  journal_ = {Computing in Science \& Engineering},
  journal = {Comput. Sci. Eng.},
  volume = {1},
  number = {1},
  pages = {42--50},
  year = {1999},
}

@INPROCEEDINGS{dabirmoghaddam:14,
  title = "{Understanding Optimal Caching and Opportunistic Caching at ``The Edge'' of Information-Centric Networks}",
  author_ = {Dabirmoghaddam, Ali and Mirzazad-Barijough, Maziar and Garcia-Luna-Aceves, Jose},
  author = {Dabirmoghaddam~\etal, Ali},
  booktitle = {Proc. ACM ICN},
  pages = {47--56},
  year = {2014},
  address = {Paris, France},
}

@BOOK{conn:00,
  title = "{Trust Region Methods}",
  author_ = {Conn, Andrew and Gould, Nicholas and Toint, P},
  author = {Conn~\etal, Andrew},
  year = 2000,
  series_ = {MPS-SIAM Series on Optimization},
  series = {MPS/SIAM S. Optimizat.},
  publisher = {SIAM},
  address_ = {Philadelphia, PA, USA},
  address = {Philadelphia, USA}
}

@ARTICLE{gratton:08,
  title = "{Recursive Trust-Region Methods for Multiscale Nonlinear Optimization}",
  author_ = {Gratton, Serge and Sartenaer, Annick and Toint, Philippe},
  author = {Gratton~\etal, Serge},
  journal_ = {SIAM Journal on Optimization},
  journal = {SIAM J. Optimiz.},
  volume = {19},
  number = {1},
  pages = {414--444},
  year = {2008},
}

@INPROCEEDINGS{dai:12,
  author_ = {Dai, Huichen and Liu, Bin and Chen, Yan and Wang, Yi},
  author = {Dai~\etal, Huichen},
  title = "{On Pending Interest Table in Named Data Networking}",
  booktitle = {Proc. ACM/IEEE ANCS},
  year = {2012},
  address_ = {Austin, TX, USA},
  address = {Austin, USA},
  pages = {211--222},
}

@INPROCEEDINGS{yuan:14,
  title = "{Scalable Pending Interest Table Design: From Principles to Practice}",
  author = {Yuan, Haowei and Crowley, Patrick},
  booktitle = {Proc. IEEE INFOCOM},
  pages = {2049--2057},
  year = 2014,
  address = {Toronto, Canada},
}

@INPROCEEDINGS{wang:12,
  title = "{Scalable Name Lookup in NDN Using Effective Name Component Encoding}",
  author_ = {Wang, Yi and He, Keqiang and Dai, Huichen and Meng, Wei and Jiang, Junchen and Liu, Bin and Chen, Yan},
  author = {Wang~\etal, Yi},
  booktitle = {Proc. IEEE ICDCS},
  pages = {688--697},
  year = {2012},
  address = {Macau, China},
}

@INPROCEEDINGS{varvello:13,
  title = "{On the Design and Implementation of a Wire-Speed Pending Interest Table}",
  author_ = {Varvello, Matteo and Perino, Diego and Linguaglossa, Leonardo},
  author = {Varvello~\etal, Matteo},
  booktitle = {Proc. IEEE INFOCOM Workshops},
  pages = {369--374},
  year = {2013},
  address = {Turin, Italy},
}

@INPROCEEDINGS{virgilio:13,
  title = "{PIT Overload Analysis in Content Centric Networks}",
  author_ = {Virgilio, Matteo and Marchetto, Guido and Sisto, Riccardo},
  author = {Virgilio~\etal, Matteo},
  booktitle = {Proc. ACM SIGCOMM Workshop on ICN},
  pages = {67--72},
  year = {2013},
  address = {Hong Kong, China},
}

@INPROCEEDINGS{abu:14,
  title = "{Interest Packets Retransmission in Lossy CCN Networks and Its Impact on Network Performance}",
  author_ = {Abu, Amuda and Bensaou, Brahim and Wang, Jason},
  author = {Abu~\etal, Amuda},
  booktitle = {Proc. ACM ICN},
  pages = {167--176},
  year = 2014,
  address = {Paris, France},
}

@INPROCEEDINGS{dehghan:15,
  author_ = {Dehghan, Mostafa and Jiang, Bo and Dabirmoghaddam, Ali and Towsley, Don},
  author = {Dehghan~\etal, Mostafa},
  title = "{On the Analysis of Caches with Pending Interest Tables}",
  booktitle = {Proc. ACM ICN},
  year = 2015,
  address_ = {San Francisco, CA, USA},
  address = {San Francisco, USA},
  pages = {69--78},
}

@ARTICLE{ioannidis:08,
  title = "{On the Design of Hybrid Peer-to-Peer Systems}",
  author = {Ioannidis, Stratis and Marbach, Peter},
  journal_ = {ACM SIGMETRICS Performance Evaluation Review},
  journal = {ACM SIGMETRICS Perform. Eval. Rev.},
  volume = {36},
  number = {1},
  pages = {157--168},
  year = {2008},
}

@INPROCEEDINGS{ioannidis:09,
  title = "{Absence of Evidence as Evidence of Absence: A Simple Mechanism for Scalable P2P Search}",
  author = {Ioannidis, Stratis and Marbach, Peter},
  booktitle = {Proc. IEEE INFOCOM},
  pages = {576--584},
  year = {2009},
  address = {Rio de Janeiro, Brazil}
}

@ARTICLE{ni:05,
  title = "{Large-Scale Cooperative Caching and Application-Level Multicast in Multimedia Content Delivery Networks}",
  author = {Ni, Jian and Tsang, Danny},
  journal_ = {IEEE Communications Magazine},
  journal = {IEEE Commun. Mag.},
  volume = {43},
  number = {5},
  pages = {98--105},
  year = {2005},
}

@INPROCEEDINGS{chand:04,
  title = "{XNET: A Reliable Content-Based Publish/Subscribe System}",
  author = {Chand, Raphael and Felber, Pascal},
  booktitle = {Proc. IEEE SRDS},
  pages = {264--273},
  year = {2004},
  address = {Florianpolis, Brazil},
}

@INPROCEEDINGS{jj-icccn:15,
  title = "{A More Scalable Approach to Content Centric Networking}",
  author = {Garcia-Luna-Aceves, J},
  booktitle = {Proc. ICCCN},
  pages = {1--8},
  year = {2015},
  address_ = {Las Vegas, NV, USA},
  address = {Las Vegas, USA}
}

@INPROCEEDINGS{jj-icnc:16,
  title = "{A Light-Weight Forwarding Plane for Content Centric Networks}",
  author = {Garcia-Luna-Aceves, J. and Mirzazad-Barijough, Maziar},
  booktitle = {Proc. IEEE ICNC},
  pages_ = {1--8},
  year = {2016},
  address_ = {Kauai, HI, USA},
  address = {Kauai, USA}
}

@INPROCEEDINGS{jj-ifip:16,
  title = "{Content-Centric Networking Using Anonymous Datagrams}",
  author = {Garcia-Luna-Aceves, J. and Mirzazad-Barijough, Maziar},
  booktitle = {Proc. IFIP Networking},
  pages_ = {1--8},
  year = {2016},
  address = {Vienna, Austria}
}
